Architecture Knowledge Representation and Communication Industry Survey

Background: The literature offers various methods for capturing software architectural knowledge (AK), including views, viewpoints, and architecture decision records (ADRs). In parallel, sustainability has gained prominence in software engineering, especially concerning software architecture. Nevertheless, practical industry reviews on these subjects seem to be lacking. Aim: In this research we aim to understand the current practice in architecture knowledge, and to explore where sustainability can be applied to address sustainability in software architecture in the future. Method: We used a survey, which utilized a questionnaire containing 34 questions and collected responses from 45 architects working at a prominent bank in the Netherlands, aimed to evaluate the practical representation and communication of architectural knowledge and sustainability. Result: Our analysis yielded two primary discoveries and several intriguing detailed results regarding how AK is captured and conveyed to diverse stakeholders. Firstly, it seems crucial to develop a new architectural element that connects various architectural features and perspectives tailored for different stakeholders. Secondly, providing clear guidance, references, and goals is essential to motivate architects to adopt Sustainable Software Engineering practices. Conclusion: After analysing the data collected through this survey, we have concluded that: a) There are no established domain-specific AK methods/tools in the financial domain. Most practitioners use domain-generic tools. b) A new architectural element that links the various architectural features and viewpoints created for various stakeholders appears to be necessary. c) There is sufficient sustainability awareness and motivation among software architects. However, what they lack are clear guidance, references, and goals to practice sustainable software engineering.

==> abstract.tex <==
Software architectural knowledge refers to the knowledge that is gained during the process of designing a software architecture, which includes the decisions made during that process\cite{babar2009software}. In the literature, several methods have been developed to represent this knowledge, including views and viewpoints, architecture decision records (ADRs), and standards like ISO 42010\cite{clements2003documenting} and the C4 Model\cite{brown2018c4}. However, for this knowledge to be effective, it is important that all relevant stakeholders share information about the architecture and how it is represented. The way this information is communicated depends on the organizational structures involved and can take various forms, such as wikis, workshops, emails, etc. Understanding how architectural knowledge is represented and communicated in professional practice is important to identify appropriate relationships that address sustainability elements in software architecture. By studying how this knowledge is represented and shared, we can gain insights into best practices for ensuring that this knowledge is effectively communicated and can be used to make informed decisions about the sustainability of software architecture.
